Effects of an Immortal Stellar Population in AGN Disks

Stars are likely embedded in the gas disks of Active Galactic Nuclei (AGN). Theoretical models predict that in the inner regions of the disk these stars accrete rapidly, with fresh gas replenishing hydrogen in their cores faster than it is burned into helium, effectively stalling their evolution at hydrogen burning. We produce order-of-magnitude estimates of the number of such stars in a fiducial AGN disk. We find numbers of order $10^{2-4}$, confined to the inner $r_{\rm cap} \sim 3000 r_s \sim 0.03\rm pc$. These stars can profoundly alter the chemistry of AGN disks, enriching them in helium and depleting them in hydrogen, both by order-unity amounts. We further consider mergers between these stars and other disk objects, suggesting that star-star mergers result in rapid mass loss from the remnant to restore an equilibrium mass, while star-compact object mergers may result in exotic outcomes and even host binary black hole mergers within themselves. Finally, we examine how these stars react as the disk dissipates towards the end of its life, and find that they may return mass to the disk fast enough to extend its lifetime by a factor of several and/or may drive powerful outflows from the disk. Post-AGN, these stars rapidly lose mass and form a population of stellar mass black holes around $10M_{\odot}$. Due to the complex and uncertain interactions between embedded stars and the disk, their plausible ubiquity, and their order unity impact on disk structure and evolution, they must be included in realistic disk models.

==> nuclides.tex <==
% $Id: nuclides.tex 385 2008-07-13 20:07:02Z efb $
% nuclides.tex
% input file with macros for nuclides

% base command
\newcommand{\nuclei}[2]{\ensuremath{\mathrm{^{#1}#2}}}

% nuclides, with most highest abundance or longest half-life as default
% for example, \carbon produces ^{12}C, \carbon[13] produces ^{13}C
%
\newcommand{\neutron}{\ensuremath{n}}
\newcommand{\nt}{\neutron}
\newcommand{\proton}{\ensuremath{p}}
\newcommand{\pt}{\proton}
\newcommand{\photon}{\ensuremath{\gamma}}
\newcommand{\hydrogen}[1][1]{\nuclei{#1}{H}}
\newcommand{\helium}[1][4]{\nuclei{#1}{He}}
\newcommand{\lithium}[1][7]{\nuclei{#1}{Li}}
\newcommand{\beryllium}[1][9]{\nuclei{#1}{Be}}
\newcommand{\boron}[1][11]{\nuclei{#1}{B}}
\newcommand{\carbon}[1][12]{\nuclei{#1}{C}}
\newcommand{\nitrogen}[1][14]{\nuclei{#1}{N}}
\newcommand{\oxygen}[1][16]{\nuclei{#1}{O}}
\newcommand{\fluorine}[1][19]{\nuclei{#1}{F}}
\newcommand{\neon}[1][20]{\nuclei{#1}{Ne}}
\newcommand{\sodium}[1][23]{\nuclei{#1}{Na}}
\newcommand{\magnesium}[1][24]{\nuclei{#1}{Mg}}
\newcommand{\aluminum}[1][27]{\nuclei{#1}{Al}}
\newcommand{\silicon}[1][28]{\nuclei{#1}{Si}}
\newcommand{\phosphorus}[1][31]{\nuclei{#1}{P}}
\newcommand{\sulfur}[1][32]{\nuclei{#1}{S}}
\newcommand{\chlorine}[1][35]{\nuclei{#1}{Cl}}
\newcommand{\argon}[1][36]{\nuclei{#1}{Ar}}
\newcommand{\potassium}[1][39]{\nuclei{#1}{K}}
\newcommand{\calcium}[1][40]{\nuclei{#1}{Ca}}
\newcommand{\scandium}[1][45]{\nuclei{#1}{Sc}}
\newcommand{\titanium}[1][48]{\nuclei{#1}{Ti}}
\newcommand{\vanadium}[1][51]{\nuclei{#1}{V}}
\newcommand{\chromium}[1][52]{\nuclei{#1}{Cr}}
\newcommand{\manganese}[1][55]{\nuclei{#1}{Mn}}
\newcommand{\iron}[1][56]{\nuclei{#1}{Fe}}
\newcommand{\cobalt}[1][59]{\nuclei{#1}{Co}}
\newcommand{\nickel}[1][58]{\nuclei{#1}{Ni}}
\newcommand{\copper}[1][63]{\nuclei{#1}{Cu}}
\newcommand{\zinc}[1][64]{\nuclei{#1}{Zn}}
\newcommand{\gallium}[1][69]{\nuclei{#1}{Ga}}
\newcommand{\germanium}[1][74]{\nuclei{#1}{Ge}}
\newcommand{\arsenic}[1][75]{\nuclei{#1}{As}}
\newcommand{\selenium}[1][80]{\nuclei{#1}{Se}}
\newcommand{\bromine}[1][79]{\nuclei{#1}{Br}}
\newcommand{\krypton}[1][84]{\nuclei{#1}{Kr}}
\newcommand{\rubidium}[1][85]{\nuclei{#1}{Rb}}
\newcommand{\strontium}[1][88]{\nuclei{#1}{Sr}}
\newcommand{\yttrium}[1][89]{\nuclei{#1}{Y}}
\newcommand{\zirconium}[1][94]{\nuclei{#1}{Zr}}
\newcommand{\niobium}[1][93]{\nuclei{#1}{Nb}}
\newcommand{\molybdenum}[1][98]{\nuclei{#1}{Mo}}
\newcommand{\technetium}[1][97]{\nuclei{#1}{Tc}}
\newcommand{\ruthenium}[1][102]{\nuclei{#1}{Ru}}
\newcommand{\rhodium}[1][103]{\nuclei{#1}{Rh }}
\newcommand{\palladium}[1][106]{\nuclei{#1}{Pd}}
\newcommand{\silver}[1][107]{\nuclei{#1}{Ag}}
\newcommand{\cadmium}[1][114]{\nuclei{#1}{Cd}}
\newcommand{\indium}[1][115]{\nuclei{#1}{In}}
\newcommand{\tin}[1][120]{\nuclei{#1}{Sn}}
\newcommand{\antimony}[1][121]{\nuclei{#1}{Sb}}
\newcommand{\tellurium}[1][130]{\nuclei{#1}{Te}}
\newcommand{\iodine}[1][127]{\nuclei{#1}{I}}
\newcommand{\xenon}[1][132]{\nuclei{#1}{Xe}}
\newcommand{\cesium}[1][133]{\nuclei{#1}{Cs}}
\newcommand{\barium}[1][138]{\nuclei{#1}{Ba}}
\newcommand{\lanthanum}[1][139]{\nuclei{#1}{La}}
\newcommand{\cerium}[1][140]{\nuclei{#1}{Ce}}
\newcommand{\praseodymium}[1][141]{\nuclei{#1}{Pr}}
\newcommand{\neodymium}[1][142]{\nuclei{#1}{Nd}}
\newcommand{\promethium}[1][147]{\nuclei{#1}{Pm}}
\newcommand{\samarium}[1][152]{\nuclei{#1}{Sm}}
\newcommand{\europium}[1][153]{\nuclei{#1}{Eu}}
\newcommand{\gadolinium}[1][158]{\nuclei{#1}{Gd}}
\newcommand{\terbium}[1][159]{\nuclei{#1}{Tb}}
\newcommand{\dysprosium}[1][164]{\nuclei{#1}{Dy}}
\newcommand{\holmium}[1][165]{\nuclei{#1}{Ho}}
\newcommand{\erbium}[1][168]{\nuclei{#1}{Er}}
\newcommand{\thulium}[1][169]{\nuclei{#1}{Tm}}
\newcommand{\ytterbium}[1][174]{\nuclei{#1}{Yb}}
\newcommand{\lutetium}[1][175]{\nuclei{#1}{Lu}}
\newcommand{\hafnium}[1][180]{\nuclei{#1}{Hf}}
\newcommand{\tantalum}[1][180]{\nuclei{#1}{Ta}}
\newcommand{\tungsten}[1][184]{\nuclei{#1}{W}}
\newcommand{\rhenium}[1][187]{\nuclei{#1}{Re}}
\newcommand{\osmium}[1][192]{\nuclei{#1}{Os}}
\newcommand{\iridium}[1][193]{\nuclei{#1}{Ir}}
\newcommand{\platnium}[1][195]{\nuclei{#1}{Pt}}
\newcommand{\gold}[1][197]{\nuclei{#1}{Au}}
\newcommand{\mercury}[1][202]{\nuclei{#1}{Hg}}
\newcommand{\thallium}[1][205]{\nuclei{#1}{Tl}}
\newcommand{\lead}[1][208]{\nuclei{#1}{Pb}}
\newcommand{\bisumth}[1][209]{\nuclei{#1}{Bi}}
\newcommand{\polonium}[1][210]{\nuclei{#1}{Po}}
\newcommand{\astatine}[1][210]{\nuclei{#1}{At}}
\newcommand{\radon}[1][222]{\nuclei{#1}{Rn}}
\newcommand{\francium}[1][223]{\nuclei{#1}{Fr}}
\newcommand{\radium}[1][226]{\nuclei{#1}{Ra}}
\newcommand{\actinium}[1][227]{\nuclei{#1}{Ac}}
\newcommand{\thorium}[1][232]{\nuclei{#1}{Th}}
\newcommand{\protactinium}[1][231]{\nuclei{#1}{Pa}}
\newcommand{\uranium}[1][238]{\nuclei{#1}{U}}
\newcommand{\neptunium}[1][237]{\nuclei{#1}{Np}}
\newcommand{\plutonium}[1][244]{\nuclei{#1}{Pu}}
\newcommand{\americium}[1][243]{\nuclei{#1}{Am}}
\newcommand{\curium}[1][247]{\nuclei{#1}{Cm}}
\newcommand{\berkelium}[1][247]{\nuclei{#1}{Bk}}
\newcommand{\californium}[1][251]{\nuclei{#1}{Cf}}
\newcommand{\einsteinium}[1][252]{\nuclei{#1}{Es}}
\newcommand{\fermium}[1][257]{\nuclei{#1}{Fm}}
\newcommand{\mendelevium}[1][258]{\nuclei{#1}{Md}}
\newcommand{\nobelium}[1][259]{\nuclei{#1}{No}}
\newcommand{\lawrencium}[1][262]{\nuclei{#1}{Lr}}
\newcommand{\rutherfordium}[1][261]{\nuclei{#1}{Rf}}
\newcommand{\dubnium}[1][268]{\nuclei{#1}{Db}}
\newcommand{\seaborgium}[1][271]{\nuclei{#1}{Sg}}
\newcommand{\bohrium}[1][274]{\nuclei{#1}{Bh}}
\newcommand{\hassium}[1][270]{\nuclei{#1}{Hs}}
\newcommand{\meitnerium}[1][278]{\nuclei{#1}{Mt}}
\newcommand{\darmstadtium}[1][281]{\nuclei{#1}{Ds}}
\newcommand{\roentgenium}[1][281]{\nuclei{#1}{Rg}}
\newcommand{\copernicum}[1][285]{\nuclei{#1}{Cn}}


==> orcid.tex <==
0000-0001-5048-9973

